The External Magnetic Field Created by the Superposition of Identical Parallel Finite Solenoids

Using superposition and numerical approximations of a published analytical expression for the magnetic field generated by a finite solenoid, we show that the magnetic field external to parallel identical solenoids can be nearly uniform and substantial, even when the solenoids have lengths that are large compared to their radii. We study two arrangements of solenoids---a ring of parallel solenoids whose surfaces are tangent to a common cylindrical surface and to nearest neighbours, and a large finite hexagonal array of parallel solenoids---and summarize how the magnitude and uniformity of the resultant external field depend on the solenoid length and distances between solenoids. We also report some novel results about single solenoids, e.g., that the energy stored in the internal magnetic field exceeds the energy stored in the spatially infinite external magnetic field for even short solenoids. These results should be broadly interesting to undergraduates learning about electricity and magnetism as novel examples of superposition based on a familiar source of magnetic fields.

==> results.tex <==
\subsection{Some New Insights About a Single Continous Solenoid}
\label{subsec:results-single-solenoid}

\begin{enumerate}
\item Discuss how $|B|$ varies with increasing $L$ for several
  representative radial values, mention the peak in $|B|(L)$ that
  Melody discovered for small~$L$.

\item Mention agreement with $1/L^2$ decrease in $|B|$ for $r \gg a$,
  in accord with Griffiths expression, discuss deviationsf rom $1/L^2$
  for near field.

\item Mention that, surprisingly, total magnetic field energy in
  external field is smaller than the internal magnetic field except
  for quite small lengths~$L$. So external field, although infinite in
  extent, stores little magnetic energy for most solenoids.

\item Discuss the singularity in~$B_r(r,z)$ as $r \to a$ for $z=\pm
  L/2$, does not occur for solenoids made out of wires with finite
  cross-section. Singularity leads to finite magnetic energy even
  though $B_r$ diverges at $r=a$ (need to verify this). Also need to
  figure out nature of singularity if possible, what is mathematical
  form of $|Br|$ as $r \to a$ from either side?
\end{enumerate}


\subsection{A Ring of Identical Parallel Solenoids}
\label{subsec:results-ring-of-solenoids}

\begin{figure}[h!]
\centering
%\includegraphics{fig1.eps}
\caption{Perspective view (a) and cross-sectional view (b) of a ring
  of identical parallel solenoids, each of radius~$a$, length~$L$,
  uniform current density~$\iota$. The solenoids are tangent to each
  other and to a central parallel cylindrical surface of radius~$1$.}
\label{fig-geometry-ring-of-solenoids}
\end{figure}

\begin{figure}[h!]
\centering
%\includegraphics{fig1.eps}
\caption{The $x$ and~$y$~components of the total magnetic field~${\bf
    B}_{\rm tot}$ at a given point~$P$ is obtained by projecting
  the~$B_r$ component at~$P$ due to the $i$th solenoid along the $x$
  and~$y$ axes as shown. }
\label{fig-projection-of-br-to-get-bx-by}
\end{figure}



\subsection{An Hexagonal Array of Parallel Identical Solenoids}
\label{subsec:results-hex-array-of-solenoids}



